Random Walk on Multiple Networks

Random Walk is a basic algorithm to explore the structure of networks, which can be used in many tasks, such as local community detection and network embedding. Existing random walk methods are based on single networks that contain limited information. In contrast, real data often contain entities with different types or/and from different sources, which are comprehensive and can be better modeled by multiple networks. To take advantage of rich information in multiple networks and make better inferences on entities, in this study, we propose random walk on multiple networks, RWM. RWM is flexible and supports both multiplex networks and general multiple networks, which may form many-to-many node mappings between networks. RWM sends a random walker on each network to obtain the local proximity (i.e., node visiting probabilities) w.r.t. the starting nodes. Walkers with similar visiting probabilities reinforce each other. We theoretically analyze the convergence properties of RWM. Two approximation methods with theoretical performance guarantees are proposed for efficient computation. We apply RWM in link prediction, network embedding, and local community detection. Comprehensive experiments conducted on both synthetic and real-world datasets demonstrate the effectiveness and efficiency of RWM.

==> GeneralMultiNetwork.tex <==
\subsection{The General Case}
\label{section:general}
In general, different networks may have different node sets. 
In this case, let the bipartite graph $G_{(i,j)}$ represent cross-network edges (or node mapping relationships) between networks $G_i$ and  $G_{j}$. Let $\mathbf{S}_{(i,j)}$ represent the transition matrix of $G_{(i,j)}$. 
Given a starting node $q$ on network $G_i$, we set $\mathbf{x}_i^{(0)}=\mathbf{e}_q$. For network $G_j$, $i \neq j$,  we initialize $\mathbf{x}_j^{(0)}$ by 
$\mathbf{x}_j^{(0)} = \mathbf{S}_{(i,j)}\mathbf{x}_{i}^{(0)}$. 

In the general case, we cannot simply merge transition matrices of different networks directly. We cannot directly compare visiting score vectors of different walkers either. To address this issue, we extend \rwm by taking advantage of bipartite graphs connecting different networks. Specifically, we define $\mathcal{P}_i^{(t)}$ as  
 \begin{equation}
 \label{eq:general_p}
      \mathcal{P}_i^{(t)} = \sum_j \hat{\mathbf{W}}^{(t)}(i,j) \mathbf{S}_{(j,i)} \mathbf{P}_j  \mathbf{S}_{(i,j)}
 \end{equation}
where $\hat{\mathbf{W}}^{(t)}(i,j) = \frac{\mathbf{W}^{(t)}(i,j)}{\sum_k\mathbf{W}^{(t)}(i,k)}$ and  $\mathbf{W}^{(t)}(i,j)$ is the local similarity score between network $G_i$ and $G_j$
at time $t$. Similarly, we design $\mathbf{W}^{(t)}(i,j)$ based on cosine similarity of their visiting histories $\mathbf{x}_{i}^{(t)}$ and $\mathbf{x}_{j}^{(t)}$. Since these two vectors are in different spaces, we map $\mathbf{x}_{j}^{(t)}$ to $\mathbf{x}_{i}^{(t)}$'s space by multiplying transition matrix $\mathbf{S}_{(j,i)}$. Thus, when $t>0$, we have
\begin{equation}
 \label{eq:general_ws}
     \mathbf{W}^{(t)}(i,j)=\mathbf{W}^{(t-1)}(i,j)+\lambda^{t} \textrm{cos} (\mathbf{x}_{i}^{(t)},\mathbf{S}_{(j,i)}\mathbf{x}_{j}^{(t)})
\end{equation}
where $\lambda \in (0,1)$ is the decay factor. Similar as in the simplified case, we initialize $\mathbf{W}^{(0)}$ by Eq. (\ref{eq:w0}).
 Since $\mathcal{P}_i^{(t)}$ is not always stochastic, we use its column-normalized version $\hat{\mathcal{P}}_i^{(t)}$ as the transition matrix for $i$\textsuperscript{th} walker at time $t$. 
 Then we have
\begin{equation}
    \label{eq:general_ite}
      \mathbf{x}_{i}^{(t+1)} = \hat{\mathcal{P}}_i^{(t)}\mathbf{x}_{i}^{(t)}% = \sum_i \hat{\mathbf{W}}^{(t)}(k,i) \mathbf{S}_{(k,i)} P^{(i)} \mathbf{S}_{(i,k)}x^{(t)}
 \end{equation}
\newadded{We present the convergence property on the transition matrix $\hat{\mathcal{P}}_i^{(t)}$ in the following Theorem.}


 \begin{theorem}
 \label{th:converge_general}
 For any small tolerance $0<\epsilon <1$, for all $i$, $\Delta(t+1) =\parallel \hat{\mathcal{P}}_i^{(t+1)}-\hat{\mathcal{P}}_i^{(t)}\parallel_\infty< \epsilon$, when $t > \lceil  \log_\lambda\frac{\epsilon}{K^2(|V_i|+2)} \rceil$, where $V_i$ is the node set of network $G_i$. 
 \end{theorem}

\begin{proof}
Refer to Appendix A.
\end{proof}
 
 
